Automated Side-Channel Analysis of Cryptographic Protocol Implementations

Formal verification of cryptographic protocols typically relies on symbolic models that abstract away compiled code and microarchitectural side channels, leaving a gap between verified specifications and deployed executables. We present a toolchain that extracts protocol-relevant models from real binaries and analyzes them under explicit leakage contracts for constant-time and Spectre-PHT-style speculative observations. Starting from a selected binary region, we lift machine code to an intermediate representation, instrument it with leakage contracts, symbolically execute it to obtain event/observation traces, and translate these traces into Sapic+ for analysis with Tamarin, ProVerif, and DeepSec. As case studies, we extract models of WhatsApp Desktop's session-management and double-ratchet components from its binary and analyze forward secrecy and post-compromise security under a state-cloning compromise. For side-channel analysis, we study the Basic Access Control (BAC) protocol used in e-passports and WhatsApp's session establishment. Under our observation models, we identify an instruction-cache side channel in WhatsApp Desktop enabling social-graph inference, and we reproduce known unlinkability issues in BAC under microarchitectural observations.

==> macros-bir.tex <==
\ProvidesPackage{macros-bir}
\newcommand{\memsymb}{\mathit{Mem}}
\newcommand{\heap}{\mathit{heap}}
\newcommand{\update}{\mathit{mstore}}
\newcommand{\memload}{\mathit{mload}}
\newcommand{\addrsymb}{\mathit{addr}}
\newcommand{\birsymb}{\fstlangcol{BIR}}
\newcommand{\sbirsymb}{\fstlangcol{SBIR}}
\newcommand{\statesymb}{\mathit{s}}
\newcommand{\envsymb}{\eta}
%%---------------------------------
\newcommand{\bnfconcat}{\!::\!}
\newcommand{\bnfsep}{\;|\;}
\newcommand{\bnfdef}{\;\;:=\;\;}
\newcommand{\bnfc}[1]{\operatorname{\textnormal{\textbf{#1}}}}
\newcommand{\domain}[1]{\mathit{dom}(#1)}
\newcommand{\imagesym}{\mathit{range}}
\newcommand{\image}[1]{\imagesym(#1)}
\newcommand{\var}[1]{\fstlangcol{#1}}
\newcommand{\symvar}[1]{{\mathit{#1}}^\sbiridx}
\newcommand{\randommem}{\var{RM}}
\newcommand{\randommemidx}[1][k]{\var{r}_{\var{#1}}}
\newcommand{\envmem}{\var{ENV}}

\newcommand{\Input}[1]{\fstlangcol{In}(#1)}
\newcommand{\Output}[1]{\fstlangcol{Out}(#1)}
\newcommand{\crypto}[1]{\fstlangcol{Cr}(#1)}
\newcommand{\event}[1]{\fstlangcol{Ev}(#1)}
\newcommand{\load}[2]{\fstlangcol{Load}(#1,#2)}
\newcommand{\store}[2]{\fstlangcol{Store}(#1,#2)}
\newcommand{\assign}[2]{\fstlangcol{Asn}(#1,  #2)}
\newcommand{\Loopsym}{\fstlangcol{{Loop}}}
\newcommand{\Loop}[1]{\fstlangcol{{loop}}(#1)}
\newcommand{\freshv}[1]{\fstlangcol{Fr}(#1)}
\newcommand{\attacker}{\mathcal{A}}
\newcommand{\oraclesym}{\mathcal{L}}
\newcommand{\oracle}[1]{\oraclesym(#1)}
\newcommand{\funevent}[1]{\mathcal{E}(#1)}
\newcommand{\impfunevent}[1]{\mathit{Ev}(#1)}
\newcommand{\funeventsym}{\mathcal{E}}
\newcommand{\reg}[1]{\mathit{r}_{#1}}
\newcommand{\simrel}[3]{#1 \sim_{_{#2}} #3}
\newcommand{\simreltraces}[4]{#1 \sim_{_{#2,#3}} #4}
%%---------------BIR---------------
\newcommand{\biridx}{\fstlangcol{\scaleto{b}{3.5pt}}}
\newcommand{\birstates}{\fstlangcol{S^\biridx}}
\newcommand{\birstate}[1]{\fstlangcol{\statesymb_{_{#1}}^\biridx}}
\newcommand{\birenv}{\fstlangcol{\envsymb^\biridx}}
\newcommand{\birpc}{\fstlangcol{pc}}
\newcommand{\birvar}{\fstlangcol{Bvar}}
\newcommand{\birval}{\fstlangcol{Bval}}
\newcommand{\birexp}{\fstlangcol{Bexp}}
\newcommand{\birprog}{\fstlangcol{P}}
\newcommand{\birprogs}{\fstlangcol{BIR}}
\newcommand{\eventsym}{o}
\newcommand{\birevent}[1]{\fstlangcol{\eventsym_{_{#1}}^\biridx}}
\newcommand{\birevents}{\fstlangcol{{\obs^\biridx}}}
\newcommand{\birprogset}{\birprog_1 , ... , \birprog_m}
\newcommand{\birproglblset}{\fstlangcol\Pi}
\newcommand{\birprobinitstates}[1]{\fstlangcol{S_{\mathit{init}}^{b,n}}}
\newcommand{\birprobinitstate}[1]{\fstlangcol{\statesymb_{\mathit{init}}^{b,n}}}
\newcommand{\birrand}{\fstlangcol\Re}
\newcommand{\sbirrand}{\Re^s}

\newcommand{\xrightarrowsgl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{}_\bl{#1}
}}
\newcommand{\starxrightarrowsgl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{}^{\bl{*}}_\bl{#1}
}}
\newcommand{\plusxrightarrowsgl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{}^{\bl{+}}_\bl{#1}
}}
\newcommand{\nxrightarrowsgl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{}^{\bl{\mi{n}}}_\bl{#1}
}}
\newcommand\stackrqarrow[2]{%
	\mathrel{\stackunder[2pt]{\stackon[4pt]{$\rightsquigarrow$}{$\scriptscriptstyle#1$}}{%
			$\scriptscriptstyle#2$}}}

\newcommand{\birtrans}[4]{#3 \xrightarrowsgl{#1}_{#2} #4}
\newcommand{\birtransstar}[4]{#3 \starxrightarrowsgl{#1}_{#2} #4}
\newcommand{\birtransmulti}[4]{#3 \plusxrightarrowsgl{#1}_{#2} #4}
\newcommand{\birtransmultin}[4]{#3 \nxrightarrowsgl{#1}_{#2} #4}
\newcommand{\birtranstclosure}[4]{#3 {\stackrqarrow{#1}{}}_{#2} #4}
\newcommand{\birexecution}{\fstlangcol{R}^\biridx}
\newcommand{\birexecutions}{\fstlangcol{R}^\biridx}
\newcommand{\birtraces}{\fstlangcol{\Traces^{\biridx}}}
\newcommand{\birtrace}{\fstlangcol{\Trace^{\biridx}}}

\newcommand{\birchannel}{\it{C}_B}


\newcommand{\conidx}{{\scaleto{c}{3.5pt}}}
\newcommand{\contraces}{\Traces^{\conidx}}
\newcommand{\contrace}{t^{\conidx}}
%%--------------SBIR---------------
\newcommand{\sbiridx}{{s}}
\newcommand{\sbirstates}{\fstlangcol{S^\sbiridx}}
\newcommand{\sbirstate}[1]{\fstlangcol{\statesymb_{#1}^\sbiridx}}
\newcommand{\sbirenv}{\fstlangcol{\envsymb^\sbiridx}}
\newcommand{\sbirpcond}{\fstlangcol\phi}
\newcommand{\sbirvals}{\fstlangcol{SE}}
\newcommand{\sbirvaluation}{\fstlangcol{H}}
\newcommand{\sbirvaluations}{\fstlangcol\mathcal{H}}
\newcommand{\sbirevent}[1]{\fstlangcol{\eventsym_{_{#1}}^\sbiridx}}
\newcommand{\sbirevents}{\fstlangcol{\obs^\sbiridx}}
\newcommand{\sbirtrace}{\fstlangcol{\Trace^{\sbiridx}}}
\newcommand{\symtraces}{\Traces^{\sbiridx}}
\newcommand{\symtrace}{t^{\sbiridx}}

\newcommand{\defeq}{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny def}}}{=}}}
\newcommand{\lbls}{L}
\newcommand{\entr}{E}
\newcommand{\pcincsym}{\mathit{ret}}
\newcommand{\pcinc}[1]{\pcincsym(#1)}
\newcommand{\transition}[2]{{#1} \rightarrow {#2}}
\newcommand{\transitions}[3]{{#1} \fstlangcol{\rightarrow}^{#2} {#3}}
\newcommand{\transitionsf}[4]{{#1} \fstlangcol{\rightarrow}^{#2}_{#3} {#4}}
\newcommand{\HLsymbexec}[3]{{#2}\rightsquigarrow_{#1}{#3}}
% \newcommand{\symmatch}[3]{#1 \mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny #2}}}{\triangleright}} #3}
% \newcommand{\symmatchext}[3]{#1 \mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny #2}}}{\blacktriangleright}} #3}

\newcommand{\xrightarrowdbl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{\mkern-14mu}\rightarrow_\bl{#1}
}}
\newcommand{\plusxrightarrowdbl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{\mkern-14mu}\rightarrow^{\bl{+}}_\bl{#1}
}}
\newcommand{\nxrightarrowdbl}[2][]{\fstlangcol{%
		\xrightarrow[]{\bl{#2}}\mathrel{\mkern-14mu}\rightarrow^{\bl{\mi{n}}}_\bl{#1}
}}
\newcommand{\sbirtrans}[4]{#3 \xrightarrowdbl{#1}_{#2} #4}
\newcommand{\sbirtransmulti}[4]{#3 \plusxrightarrowdbl{#1}_{#2} #4}
\newcommand{\sbirtransmultin}[4]{#3 \nxrightarrowdbl{#1}_{#2} #4}

\newcommand{\syminput}[1]{\bnfc{In}(#1)}
\newcommand{\symoutput}[1]{\bnfc{Out}(#1)}
\newcommand{\symcrypto}[1]{\bnfc{Cr}(#1)}
\newcommand{\symevent}[1]{\bnfc{Ev}(#1)}
\newcommand{\symfreshv}[1]{\bnfc{Fr}(#1)}
\newcommand{\sbirexecution}{\fstlangcol{R}^\sbiridx}
\newcommand{\sbirexecutions}{\fstlangcol{R}^\sbiridx}

\newcommand{\sbirprobinitstates}[1]{\fstlangcol{S_{\mathit{init}}^{s,n}}}
\newcommand{\sbirprobinitstate}[1]{\fstlangcol{\statesymb_{\mathit{init}}^{s,n}}}
\newcommand{\advmem}{\fstlangcol{\memsymb_{\mathcal{A}}}}
\newcommand{\sbiradvhistorysym}{\fstlangcol{AH}}
\newcommand{\sbiradvhistory}[1]{\sbiradvhistorysym(#1)}
\newcommand{\birtosbirvaluesym}{\delta}
\newcommand{\birtosbirvalue}[1]{\birtosbirvaluesym(#1)}
\newcommand{\sbirtoiml}[1]{\llparenthesis #1 \rrparenthesis}%_{\text{c}}



==> macros-meta.tex <==
\ProvidesPackage{macros-meta}[2024/01/29]

%%%% Meta-commands for font categories

\newcommand{\mathvar}[1]{\mathsf{#1}}
\newcommand{\mathstring}[1]{\text{\texttt{\smaller{}#1}}}
\newcommand{\mathname}[1]{\text{\textrm{#1}}}
\newcommand{\mathalg}[1]{\text{\textsc{#1}}}
\newcommand{\mathfun}[1]{{\sf #1}} 
\newcommand{\mathtext}[1]{\text{#1}}
\newcommand{\mathvalue}[1]{\mathit{#1}}
\newcommand{\mathentity}[1]{\text{\textsc{#1}}}
\newcommand{\mathnamesc}[1]{\textsc{#1}}
\newcommand{\mathlabel}[1]{\textsf{#1}}
\newcommand{\mathset}[1]{\mathname{#1}}
\newcommand{\mathsymb}[1]{\mathfun{#1}}
\newcommand{\opcode}[1]{\text{\textit{#1}}}
\newcommand{\progcmdraw}[1]{\mathsf{#1}}
\newcommand{\progcmd}[1]{\progcmdraw{#1}~}
\newcommand{\textop}[1]{\relax\ifmmode\mathop{\text{#1}}\else\text{#1}\fi}


==> macros-parallel.tex <==
\ProvidesPackage{macros-parallel}[2025/01/29]

\RequirePackage{xspace}

%%------------color------------
\newcommand{\mi}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\mr}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\mt}[1]{\ensuremath{\texttt{#1}}}
\newcommand{\mtt}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\mf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mk}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\mb}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\mtsc}[1]{\ensuremath{\mathscr{#1}}}

\newcommand{\neutcol}[0]{black}
\newcommand{\rblu}[0]{RoyalBlue}
\newcommand{\redo}[0]{RedOrange}
\newcommand{\plm}[0]{Plum}
\newcommand{\emr}[0]{Emerald}
\newcommand{\commoncol}[0]{black}    % ForestGreen

\newcommand{\col}[2]{\ensuremath{{\color{#1}{#2}}}}

\newcommand{\fstlangcol}[1]{\mf{\col{\rblu}{#1}}}
\newcommand{\sndlangcol}[1]{\ms{\col{\redo}{#1}}}
\newcommand{\trdlangcol}[1]{\mtt{\col{\plm}{#1}}}

\newcommand{\bl}[1]{\col{\neutcol }{#1}}
\newcommand{\com}[1]{\mi{\col{\commoncol }{#1}}}

\newcommand{\colone}[0]{\fstlangcol{1}}
\newcommand{\coltwo}[0]{\sndlangcol{2}}
%%-------------------------------------

\newcommand{\Sapic}{\sndlangcol{\textsc{Sapic}^+}\xspace}
\newcommand{\SapicOriginal}{\sndlangcol{\textsc{Sapic}}\xspace}
\newcommand{\SapicOld}{\sndlangcol{\textsc{Sapic}^-}\xspace}
\newcommand{\ProVerif}{\textsc{ProVerif}\xspace}
\newcommand{\CryptoVerif}{\textsc{CryptoVerif}\xspace}
\newcommand{\GSVerif}{\textsc{GSVerif}\xspace}
\newcommand{\Tamarin}{\textsc{Tamarin}\xspace}
\newcommand{\DeepSec}{\textsc{DeepSec}\xspace}
\newcommand{\Squirrel}{\textsc{Squirrel}\xspace}

\newcommand{\Nat}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\powerset}[1]{2^{#1}}

\newcommand{\lblsnormal}{\lbls_{\mathbb{N}}}
\newcommand{\lblsOp}{\lbls_{\mathit{Op}}}
\newcommand{\lblsrand}{\lbls_{\mathbb{R}}}
\newcommand{\lblssnd}{\lbls_{\mathbb{A}_s}}
\newcommand{\lblsrcv}{\lbls_{\mathbb{A}_r}}
\newcommand{\lblseve}{\lbls_{\mathbb{E}}}

\newcommand{\birpredset}{\Omega}
\newcommand{\birpred}{\omega}
\newcommand{\assert}[1]{Assert(#1)}
\newcommand{\birdedrel}{\vdash_{ _B}}
\newcommand{\birdedrelfun}[2]{#1 \birdedrel #2}
\newcommand{\silent}{\bnfc{Silent}}
\newcommand{\compose}{\fstlangcol{\bnfc{Cr}_{_C}}}
\newcommand{\decompose}{\fstlangcol{\bnfc{Cr}_{_D}}}
\newcommand{\cryptoCom}[1]{\compose(#1)}
\newcommand{\cryptoDec}[1]{\decompose(#1)}


\newcommand{\configSpace}{\calC}
\newcommand{\config}{c}
\newcommand{\stateSpace}{\tilde \calC}
\newcommand{\symbset}{\Sigma}
\newcommand{\symbSpace}{\mathcal{E}}
\newcommand{\predset}{\text{\ensuremath{\Pi}}}
\newcommand{\pred}{\varphi}
\newcommand{\predcomb}{\pred_{\colonetwo}}
\newcommand{\predSpace}{\mathcal{P}}
\newcommand{\execstate}{\mathcal{S}}
\newcommand{\dedrel}{\vdash}
\newcommand{\dedrelAvsL}{\dedrel_{\doteq}}
\newcommand{\dedrelfun}[2]{#1 \dedrel #2}
\newcommand{\xxrightarrowsgl}[2][]{{%
		\xrightarrow[]{\bl{#2}}\mathrel{}_\bl{#1}
}}
\newcommand{\nrightarrowsgl}[2][]{{%
	\centernot{\xrightarrow[]{\bl{#2}}\mathrel{}_\bl{#1}}
}}
\newcommand{\ntransrel}[4]{ #3 \nrightarrowsgl{#1}_{#2} #4}
\newcommand{\transrel}[4]{#3 \xxrightarrowsgl{#1}_{#2} #4}
\newcommand{\multransrel}[4]{#3 \xxrightarrowsgl{#1}^+_{#2} #4}

\newcommand{\eventSpaceSync}{{\mathbb{E}}_{S}}
\newcommand{\eventSpaceNonSync}{{\mathbb{E}}_{N}}
\newcommand{\PtoA}[1]{\com{P2A}(#1)}
\newcommand{\AtoP}[1]{\com{A2P}(#1)}
\newcommand{\PtoAsym}{\com{P2A}}
\newcommand{\AtoPsym}{\com{A2P}}
\newcommand{\Syncfresh}[1]{\com{SFr}(#1)}
\newcommand{\Silent}[1]{\com{Silent}(#1)}
\newcommand{\Alias}[2]{\sndlangcol{Alias}(#1,#2)}

\newcommand{\System}{S}
\newcommand{\SysFst}[1][]{\fstlangcol{\System{#1}}}
\newcommand{\SysSnd}[1][]{\sndlangcol{\System{#1}}}

\newcommand{\colonetwo}{\colone \coltwo}
\newcommand{\dedrelcomb}{\dedrel_{\colonetwo}}
\newcommand{\subone}[1]{\fstlangcol{#1_1}}
\newcommand{\subtwo}[1]{\sndlangcol{#1_2}}

\newcommand{\eqone}{\fstlangcol{\doteq}}
\newcommand{\eqtwo}{\sndlangcol{\doteq}}

\newcommand{\dycol}[1]{\sndlangcol{#1}}
\newcommand{\libcol}[1]{\trdlangcol{#1}}
\newcommand{\fstlangpred}[1]{\fstlangcol{\mathlabel{#1}}}

%\newcommand{\Term}{\calT}
\newcommand{\pubnames}{\mathcal{N}_\texttt{pub}}
\newcommand{\privnames}{\mathcal{N}_\texttt{priv}}
\newcommand{\allnames}{\mathcal{N}}
\newcommand{\Vars}{\mathcal{V}}
%\newcommand{\Funcs}{\calF}
%\newcommand{\FuncsC}{\Funcs_c}
%\newcommand{\FuncsD}{\Funcs_d}

\newcommand{\freshnesssym}{\dycol{\mathlabel{Fr}}}
\newcommand{\knowledgeset}{\dycol{\predset_{ _A}}}
\newcommand{\knowledge}[1]{\dycol{\mathcal{K}}(#1)}
\newcommand{\freshnessblue}[1]{\fstlangcol{\mathlabel{Fr}}(#1)}
\newcommand{\freshness}[1]{\dycol{\mathlabel{Fr}}(#1)}


\newcommand{\libfreshnesssym}{\libcol{\mathlabel{Fr}}}
\newcommand{\libknowledgeset}{\libcol{\predset_{ _L}}}
\newcommand{\libknowledge}[1]{\libcol{\mathcal{K}}(#1)}
\newcommand{\libfreshness}[1]{\libcol{\mathlabel{Fr}}(#1)}
\newcommand{\libstate}{\libcol{\epsilon}}

\newcommand{\fcall}[1]{\fstlangcol{{FCall}}(#1)}
%\newcommand{\ecnd}[1]{\fstlangcol{{Cnd}}(#1)}
\newcommand{\progEqual}[2]{#1 \ \fstlangcol{\doteq} \ #2}
\newcommand{\dyEqual}[2]{#1 \ \dycol{\doteq} \ #2}
\newcommand{\libEqual}[2]{#1 \ \libcol{\doteq} \ #2}
\newcommand{\Equal}[2]{#1 \doteq #2}
\newcommand{\equl}[2]{ #1 \doteq_{_{\colone}} #2}
\newcommand{\equr}[2]{ #1 \doteq_{_{\coltwo}} #2}
\newcommand{\Notequal}[2]{#1 \not\doteq #2}
\newcommand{\Patterns}{\sndlangcol{Pat}}
\newcommand{\Facts}{\sndlangcol{Fact}}
\newcommand{\substitution}{\sigma}
\newcommand{\att}{\sndlangcol{att}}
\newcommand{\attvars}{\sndlangcol{\attacker\Vars}}

\newcommand{\dydedrel}{\dycol{\vdash_{ _A}}}
\newcommand{\dydedrelfun}[2]{#1 \ \dydedrel #2}
\newcommand{\dystate}{\dycol{\epsilon}}


\newcommand{\compconfig}{\calC_{\colone \coltwo}}
\newcommand{\comppredset}{\Pi_{\colone \coltwo}}
\newcommand{\compeventSpace}{\mathbb{E}_{\colone \coltwo}}
\newcommand{\compdedrel}{\vdash_{\colone \coltwo}}
\newcommand{\compdedrelfun}[2]{#1 \compdedrel #2}
\newcommand{\comptransrel}[3]{#2 \xrightarrowdbl{#1} #3}
\newcommand{\mulcomptransrel}[3]{#2 \xrightarrowdbl{#1}^+ #3}

%\newcommand{\proj}{ \downharpoonright}
\newcommand{\proji}[1]{ #1\downharpoonright_{_{i}}}
\newcommand{\proj}[2]{ #2\!\downharpoonright_{_{#1\!}}}
\newcommand{\projl}[1]{ #1\subone{\downharpoonright}}
\newcommand{\projr}[1]{ #1\subtwo{\downharpoonright}}
\newcommand{\dedrelL}{\vdash_{ _{\colone}}}
\newcommand{\dedrelfunL}[2]{#1 \dedrelL #2}
\newcommand{\dedrelR}{\vdash_{ _{\coltwo}}}
\newcommand{\dedrelfunR}[2]{#1 \dedrelR #2}

\newcommand{\Trace}{\mathfrak{t}}
\newcommand{\Traces}{\mathcal{T}}
\newcommand{\Tracesfun}[1]{\Traces(#1)}
\newcommand{\mixtrace}{\Trace_{\colone \coltwo}}
\newcommand{\mixtraces}{\Traces_{\colone \coltwo}}
\newcommand{\sbirmixtraces}{\Traces_{\colone \coltwo}^{\sbiridx}}
\newcommand{\conmixtraces}{\Traces_{\colone \coltwo}^{\conidx}}
\newcommand{\mixtracesfun}[1]{\mixtraces(#1)}
\newcommand{\birTrace}{\Trace^{\biridx}}
\newcommand{\sbirTrace}{\fstlangcol{\Trace^{\sbiridx}}}
\newcommand{\sbirtraces}{\fstlangcol{\Traces^{\sbiridx}}}

\newcommand{\compeventsym}{\alpha_{\colone \coltwo}}

\newcommand{\Parallel}[3][~]{#2 \parallel^{#1} #3}
\newcommand{\CParallel}[2]{#1 \parallel_{c} #2}
\newcommand{\SParallel}[3][~]{#2 \parallel^{#1}_{s} #3}
\newcommand{\interleaving}[2]{#1\interleave #2}
\newcommand{\Equiv}[3]{#1 \cong_{#2} #3}

\newcommand{\DY}{\mathit{DY}}

\newcommand{\interpret}{\iota}

\newcommand{\sapicidx}{\sndlangcol{\scaleto{sp}{3.5pt}}}
\newcommand{\sapicstates}{\sndlangcol{S^\sapicidx}}
\newcommand{\sapicstate}[1]{\sndlangcol{\statesymb_{#1}^\sapicidx}}
\newcommand{\sapicTrace}{\sndlangcol{\Trace^{\sapicidx}}}
\newcommand{\sapictraces}{\sndlangcol{\Traces^{\sapicidx}}}
\newcommand{\sapicconfig}{\sndlangcol{\calC^\sapicidx}}
\newcommand{\sapicevent}{\sndlangcol{\eventsym^\sapicidx}}
\newcommand{\sapicevents}{\sndlangcol{\mathbb{E}^\sapicidx}}

\newcommand{\Infact}[1]{\tt In(#1)}
\newcommand{\Outfact}[1]{\tt Out(#1)}
\newcommand{\Frfact}[1]{\tt Fr(#1)}
\newcommand{\Kfact}[1]{\tt K(#1)}

\newcommand{\fail}{\mathsf{fail}} 

\newcommand{\dedrelcombbit}{\dedrelcomb^\mathsf{bit}} 

\newcommand{\DYLib}[1]{\textsc{DYlib}_{\bl{#1}}}

\newcommand{\silentevent}{\tau}


\newcommand{\constrans}[1]{\text{\textquotesingle{}}#1\text{\textquotesingle{}}}
